The Apiza Corpus: API Usage Dialogues with a Simulated Virtual Assistant

Virtual assistant technology has the potential to make a significant impact in the field of software engineering. However, few SE-related datasets exist that would be suitable for the design or training of a virtual assistant. To help lay the groundwork for a hypothetical virtual assistant for API usage, we designed and conducted a Wizard-of-Oz study to gather this crucial data. We hired 30 professional programmers to complete a series of programming tasks by interacting with a simulated virtual assistant. Unbeknownst to the programmers, the virtual assistant was actually operated by another human expert. In this report, we describe our experimental methodology and summarize the results of the study.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/


This package contains the IEEE Computer Society subset of the full IEEEtran
package and is intended for use with IEEE Computer Society publications.
The included version of the IEEEtran_HOWTO.pdf has been specially formatted
in IEEE Computer Society (compsoc) journal mode.


For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf_compsoc.tex, bare_jrnl_compsoc.tex.
***************************************************************************


==> sections/annotation.tex <==
\section{Corpus Annotation}
\label{sec:annotation}

%eliminate a bunch of this
%discus dimensions again-- we annotated the WoZ corpus along 4 dims
% Our research objective is to lay the groundwork for the creation of a virtual assistant designed to help programmers navigate and implement unfamiliar APIs. To that end, we examine the dialogues presented in the previous section to investigate how programmers would interact with such a system. 

We annotated the dialogue acts in the WoZ corpus along four dimensions. As described in ~\Cref{sec:background}, dialogue act annotations are needed to train virtual assistants to perform specific tasks. Different annotation schemes are needed to facilitate different functionality in a VA -- to attempt to generate a comprehensive list of all dimensions for all functionality is not in line with findings from related literature~\cite{kang2018data}.  Instead, we provide a first round of annotations as a foundation on which designers of virtual assistants can build.

\vspace{-0.2cm}
\subsection{Research Questions}

We investigated four specific research questions:

% \vspace{-0.2cm}
\begin{description}
\item[$RQ_1$] What is the composition of the corpus in terms of \textbf{illocutionary} dialogue act types?
	\vspace{0.1cm}
\item[$RQ_2$] What is the composition of the corpus in terms of \textbf{API} dialogue act types?
	\vspace{0.1cm}
\item[$RQ_3$] What is the composition of the corpus in terms of \textbf{backward-facing} dialogue act types?
	\vspace{0.1cm}
\item[$RQ_4$] What is the \textbf{traceability} of specific API components in the corpus?
\end{description}
% \vspace{-0.2cm}

% We addressed each of these research questions by annotating the conversation corpus along a different dimension. The annotation schemes are described in detail in \ref{sec:methodology}.
% We addressed each of these research questions by annotating the conversation corpus along a different dimension. The annotation schemes are described in detail in \ref{sec:methodology}.


The rationale for $RQ_1$ is to discover the conversational ``flow" of the API dialogues. An ``illocutionary'' dialogue act type describes the illocutionary intent behind an utterance e.g. distinguishing between a statement intend to inform and a statement intended to suggest future action. Annotating illocutionary DA types enables us to train a VA to identify the intention behind a user's utterance and to predict the appropriate type of response (e.g. whether to respond to a question with an answer or a follow-up question).  

The rationale for $RQ_2$ is to evaluate the domain-specific content of the API dialogues. Whereas illocutionary dialogue act types label utterances as ``questions'' or ``statements,'' API dialogue act types describe what types of API knowledge (such as functionality, usage patterns, or examples) are addressed in each utterance. As Wood~\emph{et al.}~\cite{wood2018detecting} point out, a virtual assistant must be able to identify the type of domain-specific knowledge a programmer asks about in order to respond with a relevant answer.

The rationale for $RQ_3$ is to evaluate relationships among the utterances in the API dialogues. We observed that the programmer and the wizard did not always engage in simple question-answer turn-taking. Rather, dialogues sometimes became complex, with multiple conversational ``threads'' potentially progressing in parallel. A virtual assistant should be able to track separate threads in order to draft contextually appropriate responses.

The rationale behind $RQ_4$ is to identify and track the specific API components that are addressed throughout the dialogues. We refer to this identification as ``traceability,'' borrowing the term from the related software engineering discipline~\cite{1041053}.  A virtual assistant for APIs must be able to identify the API elements relevant to a user's utterance (even when those elements are not mentioned by name).

% The rationale for $RQ_1$ is to discover the conversational ``flow" of the API dialogues. An ``illocutionary'' dialogue act type describes the illocutionary intent behind an utterance e.g. distinguishing between a statement intend to inform and a statement intended to suggest future action. Annotating illocutionary DA types enables us to train a VA to identify the intention behind a user's utterance and to predict the appropriate type of response (e.g. whether to respond to a question with an answer or a follow-up question).  

% The rationale for $RQ_2$ is to evaluate the domain-specific content of the API dialogues. Whereas illocutionary dialogue act types label utterances as ``questions'' or ``statements,'' API dialogue act types describe what types of API knowledge (such as functionality, usage patterns, or examples) are addressed in each utterance. As Wood~\emph{et al.}~\cite{wood2018detecting} point out, a virtual assistant must be able to identify the type of domain-specific knowledge a programmer asks about in order to respond with a relevant answer.

% The rationale for $RQ_3$ is to evaluate relationships among the utterances in the API dialogues. In the dialogues, we observed that the programmer and the wizard did not always engage in simple question-answer turn-taking. Rather, dialogues sometimes became complex, with multiple conversational ``threads'' potentially progressing in parallel. Utterances within a thread rely on the context of previous utterances in that same thread; for instance, the excerpts in \Cref{sec:experiment_results} each follow an individual conversational thread. A virtual assistant should be able to track separate threads in order to draft contextually appropriate responses.

% The rationale behind $RQ_4$ is to identify and track the specific API components that are addressed throughout the dialogues. This identification is related to the concept assignment problem, as it involves connecting specific software components to their relevant, natural-language concepts. We refer to this identification as ``traceability,'' borrowing the term from the related software engineering discipline~\cite{1041053}.  A virtual assistant for APIs must be able to identify the specific API elements that are relevant to a user's utterance (even when those elements are not mentioned by name) in order to make useful suggestions and engage in relevant conversation. 

\vspace{-0.2cm}
\subsection{Methodology}
\label{sec:methodology}

% \vspace{-0.1cm}
\begin{table*}[t!]
	\caption{The different dimensions along which the corpus was annotated.} 
	\centering
	\vspace{-.1cm}
	\begin{tabularx}{\textwidth}{lcXX}
		\toprule
		Dialogue Act Dimension & RQ & \multicolumn{1}{c}{Summary} & \multicolumn{1}{c}{Examples} \\
		\midrule
		Illocutionary Dialogue Act Types & 1 & Set of 14 labels describing the forward-facing illocutionary force of an utterance.& \texttt{INFORM, ELICIT-INFORM, SUGGEST, ...}  \\
		\vspace{0.1cm}
		API Dialogue Act Types & 2     & Set of 11 labels describing the API information referenced in an utterance.& \texttt{FUNCTIONALITY, PATTERNS, EXAMPLES, CONTROL FLOW, ...}  \\
		\vspace{0.1cm}
		Backward-Facing Dialogue Act Types  & 3     & Set of 6 labels describing the relationship of an utterance to a previous utterance.    & \texttt{POSITIVE, NEGATIVE, PARTIAL, ...}  \\
		\vspace{0.1cm}
		Traceability  & 4     & Set of all relevant components in an API.    & \texttt{ssh\_session, ALLEGRO\_KEY\_DOWN, ssh\_disconnect(ssh\_session session)...}  \\
		\bottomrule
	\end{tabularx}
	\label{tab:DAtypes}
	\vspace{-.1cm}
\end{table*}
% \vspace{-0.1cm}

This section details the annotation schemes used to investigate the research questions detailed above. See \Cref{tab:DAtypes} for summaries of each scheme and example labels.
% This section details the annotation schemes used to investigate the research questions detailed above, and explains how they were adapted for our API dialogue corpus. See \Cref{tab:DAtypes} for summaries of each scheme and example labels.

\vspace{-0.1cm}
\subsubsection{Segmentation}
\label{sec:segmentation}
Before assigning any labels, we first had to segment the Slack messages into individual utterances~\cite{mccowan2005ami}. The length of an utterance is variable; it may consist of a single word, or span entire paragraphs, depending on the speaker's intention. In our studies, programmers and wizards often expressed multiple intentions, responded to multiple utterances, or referenced multiple API components in the course of a single message. Therefore, it was important to segment the messages before labeling. 
% Before assigning any labels, we first had to segment the Slack messages into individual utterances. McCowan~\emph{et al.}~\cite{mccowan2005ami} emphasize that dialogue acts reflect speaker intention, and in their guide, they recommend that ``each time a new intention is expressed, you should mark a new segment.'' The length of a segment is variable; it may consist of a single word, or span entire paragraphs, depending on the speaker's intention. In our studies, programmers and wizards often expressed multiple intentions, responded to multiple utterances, or referenced multiple API components in the course of a single message. Therefore, it was important to split the messages into segments before labeling. 

Our corpus presented a unique segmenting challenge: wizards often ``presented'' verbatim chunks of documentation to the programmer. These chunks could contain several paragraphs worth of information. To segment each individual utterance of the verbatim documentation would not quite be appropriate, as they do not necessarily represent separate intentions on the part of the wizard. On the other hand, to group an entire chunk of documentation into a single segment would be too coarse grained, as wizards had the ability to purposefully include and exclude certain types of information using the documentation tool described in \Cref{sec:part}. Given that fact, we chose to segment chunks of documentation by topic (e.g. discussion of all parameters was included in a a segment, separate from discussion of the return values).

\vspace{-0.1cm}
\subsubsection{Illocutionary Dialogue Act Types}
We labeled illocutionary dialogue act types using the so-called ``AMI labels.'' The AMI corpus, presented by McCowan \emph{et al.}~\cite{mccowan2005ami}, provides a coarse-grained set of labels for illocutionary DA types that are applicable to many types of conversations.  As Gangadharaiah~\emph{et al.}~\cite{gangadharaiah2018we} point out, a useful place to start annotation is with a set of 10-20 coarse-grain labels to provide a common comparison point with other datasets, even though these annotations alone are not sufficient for industrial use.

Our methodology for annotation was straightforward: McCowan \emph{et al.}~\cite{mccowan2005ami} provide an annotation guide with detailed instructions for every DA type.  We followed this guide for every conversation, labeling each utterance with the most appropriate label.  Note that we annotated both sides of the conversations, wizard and programmer, even though a virtual assistant would only need to classify the dialogue acts of the programmer -- it would know the wizard's dialogue act types because it would have generated them.  However, we annotate both sides anyway, since we are interested in the wizards' conversation strategies and providing guidance to designers of virtual assistants.  This decision is in line with recommendations by Wood~\emph{et al.} in a study of software engineering VAs~\cite{wood2018detecting}.
% Our methodology for annotation was straightforward: McCowan~\emph{et al.}~\cite{mccowan2005ami} provide an annotation guide with detailed instructions for every DA type.  We followed this guide for every conversation, labeling each utterance with the most appropriate label.  Note that we annotated both sides of the conversations, wizard and programmer, even though a virtual assistant would only need to classify the dialogue acts of the programmer -- it would know the wizard's dialogue act types because it would have generated them.  However, we annotate both sides anyway, since we are interested in the wizards' conversation strategies and providing guidance to designers of virtual assistants on how the assistants should behave.  This decision is in line with recommendations by Wood~\emph{et al.} in a study of software engineering VAs~\cite{wood2018detecting}.

To analyze the distribution of illocutionary DA types, we compared our corpus to two others: the AMI meeting corpus~\cite{mccowan2005ami} and the WoZ debugging corpus~\cite{wood2018detecting}. The AMI corpus consists of spoken multi-party discourse in simulated meetings, while the debugging corpus consists of written dialogues between programmers and wizards completing a series of bugfixing tasks. We compared the frequencies of each illocutionary DA type in each of these corpora. The frequencies didn't account for three of the original AMI labels (STALL, FRAGMENT, and BACKCHANNEL) that were primarily relevant to spoken modalities, to allow for a more direct comparison between the AMI corpus and the WoZ corpora. 
% To analyze the distribution of illocutionary DA types, we compared our corpus to two others: the AMI meeting corpus~\cite{mccowan2005ami} and the WoZ debugging corpus~\cite{wood2018detecting}. The AMI corpus consists of spoken multi-party discourse in simulated meetings, while the debugging corpus consists of written dialogues between programmers and wizards completing a series of bugfixing tasks. We compared the frequencies of each illocutionary DA type in each of these corpora, separating the frequencies of programmers and wizards when appropriate. The frequencies didn't account for three of the original AMI labels (STALL, FRAGMENT, and BACKCHANNEL) that were primarily relevant to spoken modalities, to allow for a more direct comparison between the AMI corpus and the WoZ corpora. 

\vspace{-0.1cm}
\subsubsection{API Dialogue Act Types}
The API dialogue act types in each utterance were labeled according to the taxonomy proposed by Mallej and Robillard~\cite{maalej2013patterns}. In their work, they generated a set of 12 broad categories that may be used to classify the information types present in API documentation. Tian~\emph{et al.}~\cite{tian2017apibot} applied these label not only to API documentation, but to questions about documentation as well. By training a model on API question/answer pairs associated with these labels, they were able to achieve high performance on an API information type retrieval task.

We followed the annotation guide provided by Mallej and Robillard, which describes in detail every knowledge type and provides suggestions to resolve uncertainties. We labeled API DA types in utterances by both the wizards and the programmers, but we only labeled utterances that actually contained API information. Unlike the illocutionary DA annotation scheme, Mallej and Robillard explicitly allowed for multiple labels to be applied to a single unit. 
% To annotate API knowledge, we followed the annotation guide provided by Mallej and Robillard, which describes in detail every knowledge type and provides suggestions to resolve uncertainties. The first author followed this guide for every conversation, labeling utterances by both the wizard and the programmer. Unlike the illocutionary dialogue act annotation scheme, Mallej and Robillard explicitly allowed for multiple labels to be applied to a single unit. We only labeled API Information types in utterances which contained API information.

We found that the knowledge type that Mallej and Robillard referred to as ``NON-INFORMATION'' actually encompassed valuable information in the context of these dialogues, such as the names of functions, their parameters, and their return values. As such, we decided to rename the ``NON-INFORMATION'' class to ``BASIC.'' 

We compared the distribution of API DA types to the type distribution found in the documentation for the JDK 6 Java platform, which was one of two systems that Maalej and Robillard originally coded with API knowledge types~\cite{maalej2013patterns}. There are several substantive differences between the API usage corpus and the documentation for JDK 6: they involve different APIs using different programming languages and communicate information for different purposes. As such, the comparison between these two sources was intended to identify overall trends, rather than fine-grained distinctions. 




\vspace{-0.1cm}
\subsubsection{Backward-Facing Dialogue Act Types}
We used another layer from the AMI annotation scheme~\cite{mccowan2005ami} to capture the relationships among utterances. This layer consists of only four backward-facing dialogue act types: ``POSITIVE,'' ``NEGATIVE,'' ``PARTIAL,'' and ``UNCERTAIN.'' Each of these covers a wide range of relationship types; for instance, ``POSITIVE'' can imply agreement with a previous utterance, understanding of a previous utterance, or an attempt to provide something that the previous utterance requested.

We again followed the AMI guidelines, marking relationships among utterances.  In the AMI scheme, an utterance can only relate directly to a single prior utterance, so an annotation consisted of a single label and the ID of the related utterance. Any utterance could relate to any prior utterance by either speaker. Any utterance without a backward-facing function (e.g. an utterance starting new lines of questioning) was given a placeholder ``[NONE]'' label.


 % Note that unlike the illocutionary dialogue type annotation, not every utterance needed to be labeled with a backward-facing dialogue act type (e.g. utterances starting new lines of questioning). For these, we used a placeholder ``[NONE]'' label

In the course of annotating relationships, we found that the four backward-facing dialogue act labels did not provide enough granularity to satisfactorily capture all of the observed relationships between utterances. We noted that other dialogue act labeling schemes (such as DAMSL~\cite{Core1997CodingDW}) provide more distinction between different types of relationships (e.g. DAMSL distinguishes among ``Accept,'' ``Acknowledge,'' and ``Answer'' relationships, all of which AMI would classify as ``POSITIVE''). Therefore, we chose to add three additional labels to the original AMI set of backward-facing dialogue act type labels in order to more meaningfully evaluate the relationships that occur in our specific corpus.

The three labels that we added were ``REPEAT,'' ``FOLLOW-UP,'' and ``CONTINUE.'' The ``REPEAT'' label was used to mark repetitions, repairs, or rephrasings of a previous utterance. The ``FOLLOW-UP'' label was used to mark acts that followed up on a previous utterance, either by asking a question predicated on the utterance, or providing unprompted information or suggestions based upon the previous utterance. The ``CONTINUE'' label was intended to link contiguous utterances by one speaker that form a single question or response. For instance, Apiza would often respond to requests for documentation by sending information about parameters, return values, functionality, etc. The entire response was formed of several utterances -- it would be confusing to label each utterance as having a totally separate relationship to the original query.
% When discussing the dialogue structure, we will frequently group sets of these continuous utterances into units, which we refer to as ``contributions'' (inspired by, but distinct from Herbert Clark's notion of contributions in grounding~\cite{clark1989contributing}). 

\vspace{-0.1cm}
\subsubsection{Traceability}
The ``traceability'' annotation of specific API components was inspired by topic- and entity-labeling methodologies in NLP and SE~\cite{stoyanov2008topic,wiebe2005creating, witte2008text}. This annotation layer did not have a predefined label set per se -- rather, every component of the API could potentially be used as a label. We went through every utterance and labeled any API components that were the ``topic'' of the utterance. An API component did not need to be referenced by name to constitute a topic, and direct references to a component did not necessarily make them a topic. Rather, the decision was heavily based on context, the intention of the speaker, and the retroactive role of the component in the conversation. 

For instance, the utterance ``How do I ensure a session was successfully created?'' does not explicitly name any component of the LibSSH API -- however, the ``session'' is in reference to an \texttt{ssh\_session} struct, and the question is asked directly after a discussion of the \texttt{ssh\_new()} method. Therefore, both the \texttt{ssh\_session} struct and the \texttt{ssh\_new()} method are labeled for that utterance.

% For instance, the utterance ``How do I ensure a session was successfully created?'' does not explicitly name any component of the LibSSH API -- however, the ``session'' is in reference to an \texttt{ssh\_session} struct, so that struct is listed as component. Furthermore, this question is asked directly after a discussion of the \texttt{ssh\_new()} method. Therefore, both parties are aware that the ``successful creation'' in question relates to the usage of \texttt{ssh\_new()} and that function is also labeled.


%Get rid of this? Replace with notes on agreement. 
%Give our coding process a name and cite it, explain that it comes from another domain
%acknowledge reliability and agreement
%Explain common procedure, and is not univeral, cite evidence
%Make arguement about expert vs novice annotators
%straightforward, say that we only had one annotatey boi
%Explain that its cause we needed expert
% a lot of the time theres agreement
% Explain more that annot procedure was based on related work, coordinated with other authors
%Refer to madeline carefully
%emphasize that each annotation procedure is different

%Followed procedures, when unclear, we discussed, rather than throw annotators and get agreemennt
\begin{figure*}[t]
  \includegraphics[width=\linewidth]{figures/DAdistAll.png}
  \vspace{-.7cm}
   \caption{Frequencies of illocutionary dialogue act types in our API corpus, the debugging corpus by Wood~\emph{et al.}~\cite{wood2018detecting}, and the AMI meeting corpus\cite{mccowan2005ami}. Subfigure (a) shows programmer frequencies, while subfigure (b) shows wizard frequencies.}
  \label{fig:DAdist}
  \vspace{-.2cm}
\end{figure*} 
\vspace{-0.1cm}
\subsubsection{Note on Reliability}	

In any annotation process, it is important to consider the \emph{reliability} of the annotations, or ``the extent to which different methods, research results, or people arrive at the same interpretations or facts''~\cite{krippendorff2011agreement}. This is especially true of qualitative content analysis, in which bias, fatigue, and other factors may cause an annotator to produce unreliable results~\cite{hsieh2005three,downe1992content}.
% In any annotation process, it is important to consider the \emph{reliability} of the annotations, or ``the extent to which different methods, research results, or people arrive at the same interpretations or facts''~\cite{krippendorff2011agreement}. This is especially true of qualitative content analysis, in which an annotator's subjective interpretation of data informs his or her annotations\cite{hsieh2005three}. Bias, fatigue, and other factors may cause an annotator to produce unreliable results~\cite{downe1992content}.

There are several procedures that aim to ensure annotation reliability, but none are universally applicable. A common procedure is to measure ``reproducibility'' by asking multiple, independent annotators to annotate data, and then calculating their agreement using e.g. Cohen's kappa or Krippendorff's alpha~\cite{krippendorff2004reliability}. Agreement is typically considered to be a good indicator of reliability, but it must be interpreted in the correct context. For instance, while an alpha score of $.8$ is generally considered to indicate high reliability, it is not sufficient for applications that are ``unwilling to rely on imperfect data'' e.g. using annotations as training data for automatic annotation~\cite{craggs2005evaluating}. Furthermore, relying on agreement to gauge reliability presupposes that all annotators possess the necessary domain-specific knowledge~\cite{carletta1996assessing}. Hiring these ``expert'' annotators can be a prohibitively costly and time-consuming effort. 

A strong alternative to improve reliability is a procedure that is frequently used in the social sciences~\cite{BENGTSSON20168,spooren2010coding}, and more recently, in software engineering~\cite{wood2018detecting}. This procedure has a small number of expert annotators independently annotate a corpus. Then, the annotators collaboratively discuss and resolve all disagreements, thereby creating a single set of annotations for use in applications that are less willing to rely on imperfect data~\cite{wood2018detecting}. This method is particularly useful in ``conventional'' qualitative analysis, in which annotators do not use a predetermined set of labels.

By contrast, we performed ``directed'' qualitative analysis; that is, we annotated the corpus using predetermined sets of labels. To achieve unbiased results in this sort of analysis, Hsieh and Shannon~\cite{hsieh2005three} suggest using an ``auditing'' process, in which an expert reviewer who has not annotated the data is asked to verify that the predefined labels are applied correctly. We used a similar procedure: the first author annotated the corpus following the guidelines for existing annotation schemes for each relevant dimension. Whenever there was some ambiguity as to the correct application of an annotation scheme, the first and third authors discussed the situation and decided on a correct implementation (or, in some cases, modifications to the scheme). Although this procedure does not allow us to calculate an agreement score, the auditing process allowed us to generate ``more accurate'' annotations~\cite{hsieh2005three}.

\vspace{-0.1cm}

% What we did
% Justification
% For instance, a kappa score of $.8$ is generally considered to indicate high reliability, but is not suitable 

% In our case, we did this:
% Had a single author annotate. 
% When in doubt, conulted another author, had discussion to figure out correct application
% Also aakash helped sometimes

% This method meant that we can't establish agreement.
% However, We chose to go about it this way for a number of reasons
% * Cost and time of hiring more annotators
% * Requires some amount of expertise 
% * Throwing more annotators doesn't guarantee it'll get better results


% There are a number of threats to the validity of the annotation procedures described above, the primary threat to validity being that the corpus was annotated by a single annotator. Bias, fatigue, and inconsistency are all risks when there is a single annotator. However, due to the expertise and domain knowledge necessary to annotate these dialogues, outsourcing the annotation process was not without its own set of dangers. Other threats to validity include the modifications made to AMI relationship and API information type label sets, as well as the decision to use these label sets in the first place. 












==> sections/annotation_results.tex <==
\section{Annotation Results}
\label{sec:annotation_results}


% In this section, we discuss the results of the annotation process described above. We answer each research question separately by analyzing the label distribution for each annotation scheme and providing examples of interesting or illuminating exchanges.

In this section, we discuss the results of the annotation process described above. Before assigning any labels, we segmented the programmers' and the wizards' messages into discreet utterances, as described in \Cref{sec:segmentation}. We ultimately segmented the 1947 messages in the corpus into 3183 utterances. Programmers' messages contained 1.1 utterances on average, with 6\% containing more than one utterance. Wizards' messages contained 2.2 utterances on average, with 57\% containing more than one utterance. 

% \vspace{-0.1cm}
% \begin{table}[!h]
% 	\centering
% 	\begin{tabular}{lccc}
% 		\toprule
% 		& Wizard & Programmer & Both \# \\
% 		\midrule
% 		LibSSH & 1161 & 573      & 1734  \\
% 		Allegro & 959     & 483    & 1442  \\
% 		Both  & 2120     & 1056    & 3176  \\
% 		\bottomrule
% 	\end{tabular}
% 	\label{tab:DAdist}
% \end{table}

\vspace{-0.2cm}
%HERE FIX NUMBERS
\subsection{RQ1: Illocutionary Dialogue Act Types}

% \vspace{-0.1cm}
% We annotated the conversations using the illocutionary dialogue act labels proposed in the AMI meeting corpus. Again, the purpose of this annotation scheme is to associate each utterance with the speaker's intention. 
% The annotations of illocutionary dialogue act types 

% \begin{figure*}[t!]
% \centering
% 	\begin{subfigure}{0.47\textwidth}
% 	\centering
%   		\includegraphics[width=\linewidth]{figures/dadist2.png}
%    		\caption{Frequencies of each Illocutionary DA type used by programmers in the WoZ studies compared to those in the AMI meeting corpus. The programmers in our study asked for information and advice more frequently than the others.}
%   		\label{fig:DAdist:pro}
% 	\end{subfigure}%
% 	\hspace{2em}
% 	\begin{subfigure}{0.47\textwidth}
% 	\centering
%   		\includegraphics[width=\linewidth]{figures/dadist.png}
%    		\caption{Frequencies of each Illocutionary DA type used by wizards in the WoZ studies compared to those in the AMI meeting corpus. The wizards in our study used a higher proportion of INFORM acts and a lower proportion of ASSESS acts.}
%   		\label{fig:DAdist:wiz}
% 	\end{subfigure}
%   \label{fig:DAdist}
% \end{figure*}

% \begin{figure} h
% 	\centering
%   		\includegraphics[width=\linewidth]{figures/dadist2.png}
%    		\caption{\ \ Frequencies of Illocutionary DA types used by programmers in the WoZ studies compared to those in the AMI corpus. \ Programmers in our study mainly used ELICIT-INFORM and ELICIT-OFFER-OR-SUGGESTION acts.}
%   		\label{fig:DAdist:pro}
% 	\end{figure}%

% 	\begin{figure}
% 	\centering
%   		\includegraphics[width=\linewidth]{figures/dadist.png}
%    		\caption{\ \ Frequencies of Illocutionary DA types used by \ wizards in the WoZ studies compared to those in the AMI corpus. Wizards in our study mainly used INFORM and \ SUGGEST acts.}
%   		\label{fig:DAdist:wiz}
% 	\end{figure}

% While the exact frequencies of these two illocutionary types varied from programmer to programmer, they were the two most frequent types for all but one programmer.
% Again, this general pattern held for each individual wizard.



\Cref{fig:DAdist} shows the composition of the corpus in terms of illocutionary dialogue act labels. Programmers most frequently used dialogue acts of the ELICIT-INFORM and ELICIT-OFFER-OR-SUGGESTION illocutionary types, while wizards primarily used dialogue acts of the INFORM and, to a lesser extent, SUGGEST types. These preferences seem to reflect the task goals and the participants' different roles in the API dialogues: programmers sought to learn how to use the API, and wizards provided the desired information.
% \Cref{fig:DAdist} shows the composition of the corpus in terms of illocutionary dialogue act labels. Programmers most frequently used dialogue acts of the ELICIT-INFORM and ELICIT-OFFER-OR-SUGGESTION illocutionary types, accounting for approximately $80\%$ of all programmers' dialogue acts.  Wizards primarily used dialogue acts of the INFORM type, accounting for nearly $74\%$ of their dialogue acts. The next most common label for the wizards was SUGGEST, accounting for $13\%$ of their labels.  These preferences seem to reflect the task goals and the participants' different roles in the API dialogues: programmers sought to learn how to use the API, and wizards provided the desired information.

We compared the distribution of AMI labels in our corpus to two others: the AMI meeting corpus~\cite{mccowan2005ami} and the WoZ debugging corpus~\cite{wood2018detecting}.  As shown in \Cref{fig:DAdist}, the three corpora shared a few traits: the relatively high frequency of INFORM acts and the relative rarity of the BE-NEGATIVE, COMMENT-ABOUT-UNDERSTANDING, and ELICIT-COMMENT-ABOUT-UNDERSTANDING acts. 

% Beyond those similarities, the distributions varied substantially among the corpora. The participant role (wizard or programmer) affected the frequencies of illocutionary types in both of the WoZ corpora. Compared to the speakers in the AMI corpus, programmers in both WoZ studies used more DAs of the ELICIT-INFORM and ELICIT-OFFER-OR-SUGGESTION types and fewer of the INFORM and SUGGEST types, while the opposite was true of the wizards. These tendencies were more pronounced in the API study than the debugging study; wizards in the API study used INFORM acts nearly twice as frequently as wizards in the debugging study, and programmers used ELICIT-INFORM acts more than twice as frequently. Other differences include the relative lack of ASSESS and OFFER act types in the API corpus compared to the other corpora.
Beyond those similarities, the distributions varied substantially among the three corpora. The participant role (wizard or programmer) affected the frequencies of illocutionary types in both of the WoZ corpora. Compared to the speakers in the AMI corpus, programmers in both WoZ studies used more dialogue acts of the ELICIT-INFORM and ELICIT-OFFER-OR-SUGGESTION types and fewer of the INFORM and SUGGEST types, while the opposite was true of the wizards. These tendencies were much more pronounced in the API study than the debugging study; wizards in the API study used INFORM acts nearly twice as frequently as wizards in the debugging study, and programmers used ELICIT-INFORM acts more than twice as frequently. Other notable differences include the relative lack of ASSESS and OFFER act types in the API corpus compared to the other corpora.

We observe that the distribution of illocutionary dialogue act types in the API corpus is highly imbalanced, even when compared to that of another WoZ corpus in the software engineering domain. This imbalance has a few implications for researchers looking to build an intelligent VA for API usage. On one hand, it is more difficult to train dialogue act models on skewed datasets~\cite{doi:10.1162/089120100561737}. E.g. a classifier trained on this corpus would be unlikely to correctly identify an utterance of the OFFER type, as it would have been exposed to very few training instances of that type.  Researchers have used a number of techniques~\cite{doi:10.1162/089120100561737,wood2018detecting} to counteract the effects of imbalanced data in dialogue act modeling, but these solutions are typically poor replacements for real data.

% Researchers have previously used techniques such as downsampling~\cite{doi:10.1162/089120100561737}, oversampling, and SMOTE\cite{wood2018detecting} to counteract the effects of imbalanced data in dialogue act modeling, but these solutions are typically poor replacements for real data.

On the other hand, this imbalance means that VA designers can narrow the range of interaction types supported by a VA for API usage while still providing the desired functionality. Because a few key illocutionary DA types account for the vast majority of turns, VA designers may choose to focus on those types and group the rest into the OTHER category. Doing so would inevitably reduce the expressiveness of the dialogue system, but it would ultimately be easier to train due to the constrained state and action space~\cite{rieser2011reinforcement}.
% On the other hand, this imbalance means that VA designers can narrow the range of interaction types supported by a VA for API usage while still providing the desired functionality. Because a few key illocutionary DA types account for the vast majority of turns, VA designers may simply choose to focus on those types and group the rest into the OTHER category. Although doing so would inevitably reduce the expressiveness of the dialogue system, the dialogue system would ultimately be easier to train due to the constrained state and action space~\cite{rieser2011reinforcement}.

%  Given that e.g. the OFFER type is so rare in these API dialogues, a VA designer could simply choose not to consider that type

% The distribution of illocutionary DA types demonstrates that there are a few key types of exchanges that occur in API usage dialogues (particularly the question-answer structure observed in \Cref{sec:experiment_restuls}). 

% Intuitively, there are several illocutionary DA types that For example: although there were instances in which programmers in the API dialogues made utterances of the OFFER type (expressing their intention to perform some future action), these were extremely rare, accounting for less than .1\% of programmers' utterances.

% As we noted in \Cref{sec:experiment_results}, most of the interaction between programmers and wizards in the API dialogues consisted of question-answer pairs. By contrast, participants in the debugging study seemed to exhibit a more diverse range of behaviors, exemplified in \Cref{exc:debugging}. The illocutionary DA type distributions confirm that 

% On the other hand, this imbalance demonstrates that human-computer API usage dialogues primarily consist of just a few key illocutionary DA types. This means that VA designers can narrow the range of interaction types supported by a VA for API usage while still providing the desired functionality.

%point out how other papers make use of this

%challenges that I think are here

%More diverse set of interaction , what are open challenges


%What areas would related work be able to help, or not






%The reported distribution of labels applied to the wizards' turns was influenced by the way in which verbatim excerpts from the documentation were annotated: passages from the documentation were always annotated with the INFORM label, and they were segmented by topic, in contrast to the fine-grained segmentation applied to the extemporaneous speech. Had spans of verbatim documentation been segmented and labeled identically to regular speech, or had they been condensed into single, large segments, the wizards' label distributions would have included substantially more or fewer INFORM acts. Figure \ref{fig:DAdiff} breaks down the wizards' label distributions by total label count and by percent of turns containing each label type. 

% \vspace{-0.1cm}
% \begin{table}[h]
% 	\centering
% 	\begin{tabular}{lccc}
% 		\toprule
% 		Pattern & Support & Confidence & Lift\\
% 		\midrule
% 		A $\rightarrow$ B & .5 & .5 & .5 \\
% 		A $\rightarrow$ B & .5 & .5 & .5 \\
% 		A $\rightarrow$ B & .5 & .5 & .5 \\
% 		A $\rightarrow$ B & .5 & .5 & .5 \\
% 		A $\rightarrow$ B & .5 & .5 & .5 \\
% 		\bottomrule
% 	\end{tabular}
% 	\label{tab:DApatterns}
% \end{table}
% \vspace{-0.1cm}

% We used an implementation of the Spade algorithm~\cite{Zaki:2001:SEA:599609.599626} to find frequent patterns of dialogue act types, examining sequential patterns of contributions. As described in \Cref{sec:annotation}), an utterance and all subsequent continuations were considered to be a single ``contribution'', and relationships between contributions formed sequences.  If two separate contributions had relationship pointers to the same prior itemset, they formed separate sequences. 

% The 10 most frequent sequential patterns are summarized in \Cref{tab:DApatterns}. Variations of the {ELICIT-INFORM} $\rightarrow$ {INFORM and ELICIT-OFFER-OR-SUGGESTION $\rightarrow$ SUGGEST adjacency pairs are by far the most common patterns in the dataset, corresponding to typical question/answer pairs. The next most common patterns are the reverse: SUGGEST/INFORM $\rightarrow$ ELICIT-INFORM/ELICIT-OFFER-OR-SUGGESTION. 



\vspace{-0.2cm}
\subsection{RQ2: API Dialogue Act Types}
\label{sec:api_inf}

% \vspace{-0.1cm}
\begin{figure}[t]
  \includegraphics[width=\linewidth]{figures/APIdist.png}
  \vspace{-.6cm}

   \caption{Frequencies of API dialogue act types in our API corpus and the documentation for JDK 6~\cite{maalej2013patterns}}
  \vspace{-.1cm}

  \label{fig:APIdist}
\end{figure}
% \vspace{-0.1cm}

% \vspace{-0.1cm}
\begin{figure}[t]
  \includegraphics[width=\linewidth]{figures/BFdist.png}
  \vspace{-.8cm}

   \caption{Frequencies of backward-facing dialogue act types in our API corpus.}
  \vspace{-.4cm}

  \label{fig:BFdiff}
\end{figure}
% \vspace{-0.1cm}

We annotated 2826 utterances with API dialogue act types across 1790 messages. 94\% of programmers' messages and 91\% of wizards' messages were labeled with at least one API DA type.

 % The total distribution of API DA labels assigned by participant and by library is summarized below:

% \vspace{-0.1cm}
% \begin{table}[h]
% 	\centering
% 	\begin{tabular}{lccc}
% 		\toprule
% 		& Wizard & Programmer & Both \# \\
% 		\midrule
% 		LibSSH & 754 & 515      & 1269  \\
% 		Allegro & 804     & 450    & 1254  \\
% 		Both  & 1558     & 965    & 2523  \\
% 		\bottomrule
% 	\end{tabular}
% 	\label{tab:APIdist}
% \end{table}
% \vspace{-0.1cm}


\Cref{fig:APIdist} shows the composition of the corpus in terms of API dialogue act labels. Programmers most frequently asked for information about PATTERNS (accounting for nearly half of their utterances), describing \textit{how} to accomplish a specific objective with the API, followed by queries about BASIC information and FUNCTIONALITY details.  Wizards referenced the same three API types most frequently, but the distribution differed: BASIC information was present in about 30\% of the wizards' utterances, FUNCTIONALITY in about 25\%, and PATTERNS in about 20\%. 

%See sec blah blah or cite java doc annotations FROM 
Overall, the distribution of API dialogue act types was somewhat similar to that of the JDK documentation~\cite{maalej2013patterns}, with a few notable exceptions. Compared to documentation, the dialogues contained a much higher proportion of PATTERN information, and a much smaller proportion of PURPOSE and CONTROL information. The rest of the labels followed a few trends in both the documentation and the corpus: FUNCTIONALITY, BASIC, and STRUCTURE information appeared fairly frequently, while the QUALITY, REFERENCES, and ENVIRONMENT types were rare. 

% Again, we observe an imbalanced distribution of API DA types. This imbalance presents researchers with challenges and opportunities similar to those discussed in RQ1. Specifically, while it would be difficult to train ML models on this skewed dataset, VA designers may choose to provide functionality for only the most common API DA types. 

%QA systems
%Ways to solve this: generate synthetic questions


% \cite{Agrawal:1994:FAM:645920.672836}
% We again used the Spade algorithm to mine sequential patterns. For API information types, we were not only interested in sequential patterns, but in patterns within itemsets as well; to mine those, we used the Apriori algorithm\cite{Agrawal:1994:FAM:645920.672836}. Itemsets and sequences were defined as in RQ1. The top-10 frequent patterns are:

% \vspace{-0.1cm}
% \begin{table}[h]
% 	\caption{Frequnt patterns in the sequence of DA types.} 
% 	\centering
% 	\begin{tabular}{lccc}
% 		\toprule
% 		Pattern & Support & Confidence & Lift\\
% 		\midrule
% 		A $\rightarrow$ B & .5 & .5 & .5 \\
% 		A $\rightarrow$ B & .5 & .5 & .5 \\
% 		A $\rightarrow$ B & .5 & .5 & .5 \\
% 		A $\rightarrow$ B & .5 & .5 & .5 \\
% 		A $\rightarrow$ B & .5 & .5 & .5 \\
% 		\bottomrule
% 	\end{tabular}
% 	\label{tab:APIpatterns}
% \end{table}
% \vspace{-0.1cm}


\vspace{-0.2cm}
\subsection{RQ3: Backward-Facing Dialogue Act Types}
\label{sec:relationships}



%HERE
% We used another layer of the AMI annotation scheme to label the backward-facing dialogue act types. 

\Cref{fig:BFdiff} shows the the distribution of backwards-facing dialogue act types used by the wizard and the programmer. The majority of the programmers' dialogue acts were assigned the NONE label (meaning they did not have a direct relationship to any previous utterance) or the FOLLOW-UP label. The PARTIAL, NEGATIVE, and UNCLEAR tags saw minimal use by the programmers. The majority of the wizards' dialogue acts were assigned the CONTINUE label, primarily due to the segmentation method used for verbatim chunks of documentation. The next most frequent label was POSITIVE, and the least frequent labels were START and REPAIR. These distributions demonstrate that many programmer-wizard interactions took place in the context of previous utterances. Oftentimes, the wizard relied on this context to produce an appropriate response. The following excerpt demonstrates one such situation:

\vspace{-0.2cm}
\begin{excerpt}
\begin{tcolorbox}[left=5pt,right=-18pt,top=5pt,bottom=5pt]
\begin{flushleft}
\begin{dialogue}
\speak{PRO} Apiza, what is the command to create a new ssh\_session in the libssh API?
\vspace{0.1cm}
\speak{WIZ} The command to create a new ssh session is: ssh\_session ssh\_new(void) [...] Returns A new ssh\_session pointer, NULL on error.
\vspace{0.1cm}
\speak{PRO} Just to confirm, is the ssh\_session type a pointer type?
\vspace{0.1cm}
\speak{WIZ} ssh\_session is not a pointer type.
\vspace{0.1cm}
\speak{PRO} But when you gave me the command to create a new ssh session, you said it "Returns" "A new ssh\_session pointer...". I'm confused.
\vspace{0.1cm}
\speak{WIZ} ssh\_new returns a pointer to type ssh\_session
\end{dialogue}
\end{flushleft}
\end{tcolorbox}
\label{exc:bouncy}
\end{excerpt}
\vspace{-0.3cm}


In that exchange, the wizard needed to recall the context of the method \texttt{ssh\_new} as well as the question ``is the ssh\_session type a pointer type'' in order to rectify the programmer's confusion. Furthermore, programmers did not necessarily respond to the wizard's most recent message; 16\% of programmers' backward-facing dialogue acts were related older to messages in the conversation. 
% The key take-away is that programmers naturally engaged in threads of conversation, occasionally in parallel.

%This observation, that programmers and wizards frequently relied on conversational context, underscores the need for a virtual assistant to be able to keep track of this context as well. 	

\vspace{-0.1cm}
\subsection{RQ4: Traceability}

In total, we identified 157 specific API components across 2430 utterances. The wizards referred to specific API components more often than the programmers, and a slightly broader range of API components were identified in the Allegro scenario than in the LibSSH scenario. The total number of API component labels and number of unique component labels annotated are shown below:
% In total, we identified 96 specific API components that were discussed across 1513 utterances. The wizards referred to specific API components more often than the programmers, and a broader range of API components were identified in the Allegro scenario than in the LibSSH scenario. The total number of API component labels and number of unique component labels annotated by library and by speaker are shown below:

\vspace{-0.2cm}
\begin{table}[h]
	\centering
	\begin{tabular}{llccc}
		\toprule
		 Library & Variable & Programmer & Wizard & Both \\ 
		\midrule
		\multirow{2}{*}{LibSSH}& \# Labels & 383 & 1053      & 1436  \\
		& \# Distinct labels & 41     & 74    & 76  \\
		\midrule
		\multirow{2}{*}{Allegro}& \# Labels & 343 & 922      & 1265  \\
		& \# Distinct labels & 47     & 80    & 81  \\
		\midrule
		\multirow{2}{*}{Both}& \# Labels & 726 & 1975      & 2701  \\
		& \# Distinct labels & 88     & 154    & 157  \\
		\bottomrule
	\end{tabular}
\end{table}
\vspace{-0.3cm}

% The complete traceability between API components and utterances is available in the online appendix for use by future researchers. 

%This traceability will aid in the development of QA systems. It may also be used to generate a synthetic question/answer dataset using neural approaches such as those proposed by Xu~\emph{et. al}\cite{Xu2018Graph2SeqGT}.

% \vspace{-0.1cm}
% \begin{table}[b]
% 	\caption{The most common API components discussed in each library, and the word tokens most frequently associated with them.} 
% 	\centering
% 	\begin{tabularx}{\columnwidth}{lccX}
% 		\toprule
% 		Library & API Component & \# Utterances& Related tokens\\
% 		\midrule
% 		\multirow{5}{*}{LibSSH}&A&$100$&AAAAA, BBBBB, CCCCC\\
% 		&A&$100$&AAAAA, BBBBB, CCC, fdsfdsf dsfsdCC\\
% 		&A&$100$&AAAAA, BBBBB, CCCCC\\
% 		&A&$100$&AAAAA, BBBBB, CCCCC\\
% 		&A&$100$&AAAAA, BBBBB, CCCCC\\
% 		\midrule
% 		\multirow{5}{*}{Allegro}&A&$100$&AAAAA, BBBBB, CCCCC\\
% 		&A&$100$&AAAAA, BBBBB, CCCC, fdsfdsf dsC\\
% 		&A&$100$&AAAAA, BBBBB, CCCCC\\
% 		&A&$100$&AAAAA, BBBBB, CCCCC\\
% 		&A&$100$&AAAAA, BBBBB, CCCCC\\
% 		\bottomrule
% 	\end{tabularx}
% 	\label{tab:traceability}
% \end{table}
% \vspace{-0.1cm}




























==> sections/background.tex <==
\section{Background and Related Work}
\label{sec:background}

This section discusses background on the problem we target, supporting technologies, and related work.

\vspace{-0.1cm}
\subsection{Problem, Significance, Scope}
\label{sec:prob}

The problem we target in this paper is that the composition and patterns of dialogue acts is not known for conversations between programmers and virtual assistants during API usage tasks.  This problem is significant because information about these dialogue acts must be known in order to create lifelike virtual assistant systems.  The situation is a ``chicken or egg'' question because in order to obtain the dialogue act structure, one must have conversations between programmers and VAs, but to have a VA one must know the dialogue act structure.  Software engineering literature does not describe these dialogue acts for API usage conversations, which impedes development of usable VAs.

Reiser and Lemon provide an excellent summary of the state-of-the-art in VA development in their recent book~\cite{rieser2011reinforcement}.  In short, they explain that a highly-effective method to kick start development of VAs is to conduct Wizard of Oz (WoZ) experiments to collect conversations between humans and (simulated) VAs.  The data from those experiments can then be used to design a VA prototype.  Later, as more people interact with the VA, real-world data can be collected.  As mentioned in the previous section, the process boils down to collecting WoZ data and annotating the dialogue acts in that data.

There is a temptation to jump as soon as possible to training machine learning algorithms based on whatever data are available.  This temptation should be resisted because the data collected to train a VA to do one task are generally not usable for training the VA to do other tasks.  While one hopes that it would be possible to annotate a dataset once and train a VA for many different tasks, in fact it is necessary to re-annotate data based on task-specific criteria.  Nevertheless, as Tenbrink~\emph{et al.}~\cite{tenbrink2013annotation} point out, different tasks often share similar high-level dialogue act types, from which low-level, more detailed dialogue acts can be derived.
% There is a temptation to jump as soon as possible to training machine learning algorithms based on whatever data are available.  This temptation should be resisted because the data collected to train a VA to do one task are generally not usable for training the VA to do other tasks.  While one hopes that it would be possible to annotate a dataset once and train a VA for many different tasks, in fact it is necessary to re-annotate data based on task-specific criteria.  The different components of a task must be understood before a VA can be designed to assist.  For example, in API usage, different tasks could be obtaining usage code examples, or explaining rationale behind code, or determining if an API function has changed since last used.  Different annotations and training data must be obtained for each of these tasks.  Nevertheless, as Tenbrink~\emph{et al.}~\cite{tenbrink2013annotation} point out, different tasks often share similar high-level dialogue act types, from which low-level, more detailed dialogue acts can be derived.

 % The different components of a task must be understood before a VA can be designed to assist. 

The scope of this paper is to lay groundwork for building VAs for API usage in the future.  We 1) conduct WoZ experiments, 2) annotate the conversations with high-level dialogue act types, semantic content, and utterance relationships that are likely to be useful for many tasks, and 3) discuss the key tasks within API usage that occur in our data to suggest what detailed training should be conducted in future work.  This scope is already quite extensive, so we note that we do not yet attempt automatic classification of dialogue acts, training of VAs for strategy, or natural language generation.%  Our sincere hope is that our work will propel advances in VA technology in software engineering.

\vspace{-0.2cm}
\subsection{Wizard of Oz Experiments}
\label{sec:woz}

A ``Wizard of Oz'' (WoZ) experiment is one in which a human (the user) interacts with a computer interface that the human believes is automated, but is in fact operated by another person (the wizard)~\cite{dahlback1993wizard}.  The purpose of a WoZ experiment is to collect conversation data unbiased by the niceties of human interaction: people interact with machines differently than they do with other people~\cite{schatzmann2007agenda}.  These unbiased conversation data are invaluable for kickstarting the process of building an interactive dialogue system, as discussed above. We direct readers to a comprehensive survey by Riek~\emph{et al.}~\cite{riek2012wizard} for further justification and examples of WoZ experiments.

%Refer to dimensions //more throgouhg

In a WoZ study, researchers must provide the user and the wizard with some specific \emph{scenario}. A scenario is "a task to solve whose solution requires the use of the system, but where there does not exist one single correct answer"~\cite{dahlback1993wizard}. A well-designed scenario promotes interaction relevant to the simulated system~\cite{1374824}. To that end, it is important for the scenario to place constraints on both the user and the wizard. Such constraints may include limitations on the resources available to the user, or the types of responses the wizard can generate. At the same time, the scenario should be as realistic as possible given the human limitations of the wizard~\cite{fraser1991simulating}. Researchers often provide the wizard with an interface that simplifies and expedites the process of generating a response~\cite{Lu:2011:PWO:1957656.1957729, Klemmer:2000:SWO:354401.354406}.

The WoZ technique enables researchers to rapidly prototype and evaluate different system features or characteristics. Kelley~\cite{kelley1984iterative} describes how researchers can use these simulations in an iterative design process, in which the wizard is gradually phased out as the simulated functionality is added in.  Reiser and Lemon~\cite{rieser2011reinforcement} examine subjective feedback solicited from users to determine if different wizard ``strategies'' (see \emph{Dialogue Acts} below) are more or less effective. This feedback also serves as a baseline against which future iterations of a system can be compared.


\vspace{-0.2cm}
\subsection{Dialogue Acts}

A ``dialogue act'' (DA) is a spoken or written act that accomplishes a specific purpose in a conversation, as introduced above.  DAs are typically viewed as classes into which utterances can be categorized~\cite{kumar2018dialogue, chen2018dialogue}, such as greeting or information-elicitation. 

A single dialogue act can perform multiple functions in a conversation simultaneously: for instance, the utterance ``I have to work tonight'' in response to an invitation functions as an informative act and as a rejection of the previous utterance. Dialogue act annotators can choose to provide separate labels for each relevant \emph{dimension} of a DA, or they can use a one-dimensional annotation scheme that accounts for all relevant functional combinations~\cite{popescu2005dialogue}. Most popular DA annotation schemes provide anywhere from 3 to 10 different functional dimensions~\cite{Core1997CodingDW, ISOStandard2017, DIT}. It is typical for researchers to select a subset of functions or dimensions that are most suited to their particular research problem~\cite{zarisheva2015dialog, ohtake2009annotating, chowdhury-etal-2016-transfer}.

A key observation is that there is a difference between the \emph{strategy} involved in a conversation and the \emph{language} used by people to implement that strategy~\cite{he2018decoupling}, even though a recent trend has been to train ML algorithms both strategy and language at the same time~\cite{li2016deep, lewis2017deal}.  The language is represented as the actual words used to render an utterance, while the strategy is represented as the sequence of DAs used.  E.g., the language ``A: Hello.  B: Hi.  A: Where should we eat?  B: At Joe's.'' versus the conversation flow/strategy: greeting, greeting, suggestion-elicitation, suggestion.

To create a dialogue system, both language and DA types must be known for utterances in example conversations~\cite{rieser2011reinforcement}.  A VA must learn to mimic good strategies in terms of DA flow (e.g. it must recognize that it should respond to a suggestion-elicitation with a suggestion).  Once it knows that it should respond with a particular DA type (e.g. a suggestion), it must then collect the information to portray in an utterance (e.g. a restaurant to recommend) and then convert the information into an understandable utterance in natural language.  As Serban~\emph{et. al}~\cite{serban2015survey} point out in a recent survey, several datasets, especially involving WoZ studies, have been created for a variety of domains to serve as starting points for training VAs.

\vspace{-0.2cm}
\subsection{Related Work in Software Engineering}

%//more throough analysis --- detail dimensions and stuff -- be clear what is more throughgh
Related work in the software engineering (SE) literature can be broadly categorized as either supporting experimentation or prototype virtual agents.  In terms of supporting experimentation, recent work at FSE'18~\cite{wood2018detecting} is the most similar to this paper.  In that work, the authors conducted WoZ studies for debugging tasks and built an automated classifier for DA types.  However, the one-dimensional DA annotations in that study were still rather general, such as ``statement'' or ``apiQuestion.''  This paper is different in that we have entirely new WoZ experiments for API usage and provide more thorough analysis by annotating additional dimensions of each dialogue act.  Work by Maalej~\emph{et. al}~\cite{maalej2013patterns} is also key supporting experimentation, in that it explores what types of information programmers are provided in API documentation.  Many recent experiments have been reported in a similar vein, including \cite{meng2018application, aghajani2018large, head2018not, maalej2014comprehension, monperrus2012should, robillard2011field}.

Prototype virtual agents are less common, but include APIBot~\cite{tian2017apibot}, WhyLine~\cite{ko2004designing}, TiQi~\cite{pruski2015tiqi}, and Devy~\cite{bradley2018context}.  A comprehensive survey was recently conducted by Arnaoudova~\emph{et. al}~\cite{arnaoudova2015use}.  We view our work as complementing and enhancing this work on VAs in SE.

This work follows a history of empirical studies in software engineering~\cite{Weiser:1981:PS:800078.802557, 87283,DYBA2008833, murphy2019developers}. SE researchers have successfully employed a wide variety of empirical methods, such as controlled experimentation, interviews, and case studies ~\cite{1027796, 799955,Easterbrook2008}. In their ``roadmap'' to empirical studies, Perry~\emph{et. al}~\cite{Perry:2000:ESS:336512.336586} emphasize that ``empirical studies can be used not only retrospectively to validate ideas after they've been created, but also proactively to direct our research.''

% \vspace{-0.1cm}













==> sections/experiment_results.tex <==
\section{Experiment Results}
\label{sec:experiment_results}

In this section, we present the key experimental results of our WoZ studies. We outline the basic structure and statistics of the collected dialogues, and briefly examine the programmers' task performance and satisfaction with the simulated system.


\vspace{-0.1cm}
\subsection{Dialogues}
\label{sec:dialogues}

% \vspace{-0.1cm}
% \begin{table}[h]
% 	\begin{tabular}{lccc}
% 		\toprule
% 		 & Wizard & Programmer & Both \# \\ 
% 		\midrule
% 		LibSSH & 491 & 536      & 1027  \\
% 		Allegro & 463     & 457    & 920  \\
% 		Both  & 954     & 993    & 1947  \\
% 		\bottomrule
% 	\end{tabular}
% 	\label{tab:diadist}
% \end{table}
% \vspace{-0.1cm}

We collected 30 API usage dialogues. In general, the programmer and the wizard sent messages in turn. Most frequently, these were question-answer pairs, with the programmer querying some functionality of the API and the wizard providing the answer. Other types of interactions occurred as well, such as greetings, assessments, and side-exchanges -- these are explored in greater detail in \Cref{sec:annotation_results}. The following excerpt typifies the interactions that occurred in the dialogues. Messages are labeled with ``PRO'' or ``WIZ'', denoting the speaker as a ``Programmer'' or ``Wizard,'' respectively.

\vspace{-0.2cm}
\begin{excerpt}
% \caption{An excerpt from the beginning of a study using the Allegro library. This exchange demonstrates the typical question-answer dialogue structure. Messages are labeled with ``P'' or ``W'', denoting the speaker as a ``Programmer'' or ``Wizard,'' respectively}
\begin{tcolorbox}[left=5pt,right=-15pt,top=5pt,bottom=5pt]
\begin{flushleft}
\begin{dialogue}
\speak{Pro} allegro keyboard input
\vspace{0.1cm}
\speak{Wiz} You can save the state of the keyboard specified at the time the function is called into the structure pointed to by \texttt{ret\_state}, using \texttt{al\_get\_keyboard\_state}
\vspace{0.1cm}
\speak{Pro} Whats the function signature for \texttt{al\_get\_keyboard\_state} 
\vspace{0.1cm}
\speak{Wiz} \texttt{void al\_get\_keyboard\_state( ALLEGRO\_KEYBOARD\_STATE *ret\_state)}
\end{dialogue}
\end{flushleft}
\end{tcolorbox}
\label{exc:basic}
\end{excerpt}
\vspace{-0.3cm}

Across all dialogues, participants collectively generated 1927 Slack messages (also referred to as ``turns''). Wizards and programmers sent similar quantities of messages, averaging to 31.8 messages/dialogue sent by programmers and 33.1 messages/dialogue sent by wizards. The frequency was also similar across the two tasks; participants sent an average of 68.5 messages in studies using LibSSH, compared to 61.3 sent in studies using Allegro.

The dialogues contain a total of 47928 word tokens\footnote{Word tokens were generated using the \texttt{word\_tokenize} method from Python's \texttt{nltk.tokenize.punkt} module.} with a vocabulary size of 3190 words. Wizards used considerably more words (41185) and drew from a larger vocabulary (2988) than programmers, who used 6743 words and 880 unique words. This disparity in word usage is to be expected; programmers manually wrote the majority of their messages' content, and had access to only limited information. By contrast, wizards frequently copied and pasted large chunks of pre-written documentation to send to the user.

This corpus is similar in size to published WoZ corpora across a broad range of domains, as shown in the table below:

\vspace{-0.1cm}
\begin{table}[h!]
	% \caption{Comparison of our corpus to other WoZ data sets.} 
	\centering
	\begin{tabularx}{\linewidth}{Xcccc}
		\toprule
		\multirow{2}{*}{Task Domain}&\# of&\# of&\# of &\# Unique\\
		&Dialogues&Turns&Words&Words\\
		\midrule
		APIs (this paper)&$30$&$1947$&$47928$&$3190$\\
		Debugging~\cite{wood2018detecting}&$30$&$2243$&$50514$&$4162$\\
		Design~\cite{pineda2002dime}&$31$&$3606$&$27459$&--\\
		% General QA~\cite{bertomeu2006contextual}&$33$&$2534$&$125534$&--\\
		Audio player~\cite{rieser2005corpus}&$72$&$1772$&17076&--\\
		Tutoring~\cite{benzmuller2006corpus}&$37$&$1917$&$12346$&--\\
		Mission planning~\cite{frames}&$22$&$1738$&--&--\\
		\bottomrule
	\end{tabularx}
	\label{tab:DAtypes}
\end{table}
\vspace{-0.2cm}


\vspace{-0.2cm}
\subsection{Observations}

We made a number of observations regarding the dialogues. First, we found that the programmers had generally favorable opinions of Apiza, as evidenced by their responses to the user satisfaction survey. They were particularly impressed by the system's ability to comprehend their messages. Programmers indicated that Apiza's biggest weakness was its slow response time.  Due to space limitations, we make all survey results available in our online appendix. We would like to emphasize that these results will allow researchers to evaluate wizard strategies, as well as train reinforcement learning algorithms for non-simulated dialogue systems (see \Cref{sec:woz}).
% We made a number of observations regarding the dialogues. First, we found that the programmers had generally favorable opinions of Apiza, as evidenced by their responses to the user satisfaction survey. They were particularly impressed by the system's ability to comprehend their messages.  Many programmers enjoyed testing the system's capabilities, going so far as to ask out-of-domain questions like ``How's it going?'' and ``How is the weather?'' Programmers indicated that Apiza's biggest weakness was its response time. As one programmer put it, ``the wait was a bit annoying. I'm used to getting answers within a few seconds.''  Due to space limitations, we make all survey results available in our online appendix. We would like to emphasize that these results will allow researchers to evaluate wizard strategies, as well as train reinforcement learning algorithms for non-simulated dialogue systems (see \Cref{sec:woz}).

Second, we observed that not every programmer attempted or completed every task. We considered a programmer to have ``attempted'' a task if he or she wrote at least one line of code directly related to the task. We considered a programmer to have ``completed'' a task if, in our judgment, he or she wrote all of the code to satisfy all of the task's requirements. The following table shows programmers' attempt and completion rates for each task. For instance, $71.4\%$ of all programmers attempted Task D of the LibSSH scenario; of those programmers, $40.1\%$ completed the task.
% Second, we observed that not every programmer attempted or completed every task. We considered a programmer to have ``attempted'' a task if he or she wrote at least one line of code directly related to the task. If the relationship was ambiguous, we referred to the dialogue for context. We considered a programmer to have ``completed'' a task if, in our judgment, he or she wrote all of the code to satisfy all of the task's requirements. The following table shows programmers' attempt and completion rates for each task. For instance, $71.4\%$ of all programmers attempted Task D of the LibSSH scenario; of those programmers, $40.1\%$ completed the task.

\vspace{-0.1cm}
\begin{savenotes}
	\begin{table}[h!]
	% \caption{Programmers' performance on the tasks. ``Attempt rate'' refers to the percentage of all programmers that wrote at least one line code directly related to the task. ``Success rate'' refers to the percentage of all programmers that successfully completed the task.}
		\centering
		\begin{tabular}{lcrr}
			\toprule
			Scenario & Task                & Attempt Rate (\%)              & Completion Rate (\%)\\ 
			\midrule
			\multirow{5}{*}{LibSSH\footnote{Only 14 studies are considered here, as one participant in the LibSSH studies did not submit a source code file.}}&A&$100.0$&$100.0$\\
			&B&$100.0$&$78.6$\\
			&C&$100.0$&$21.4$\\
			&D&$71.4$&$40.1$\\
			&E&$51.1$&$28.0$\\
			\midrule
			\multirow{7}{*}{Allegro}&A&$100.0$&$73.3$\\
			&B&$93.3$&$78.6$\\
			&C&$80.0$&$33.4$\\
			&D&$40.0$&$66.8$\\
			&E&$6.7$&$100.0$\\
			&F&$6.7$&$100.0$\\
			&G&$0.0$&N/A\\
					\bottomrule
		\end{tabular}
		\label{tab:performance}
	\end{table}
\end{savenotes}{}
\vspace{-0.1cm}

More information about task completion for each individual programmer is available in our online appendix. Task completion is another metric that may help future researchers to train and evaluate novel dialogue systems.
% More information about task completion for each individual programmer is available in our online appendix. As with the user satisfaction ratings, task completion is a metric that may help future researchers to train and evaluate novel dialogue systems.


Third, we observed that programmers demonstrated habits that they may have learned by interacting with other VAs and tools. Several programmers avoided the use of pronouns to refer to recently mentioned API components. They may have wanted to be as clear as possible in case Apiza was unable to resolve the antecedent. Some programmers treated Apiza like a search engine, querying vagues terms without specifying the type of information desired. Many exhibited the ``Google Effect''~\cite{Sparrow776}, asking for previously established pieces of information (even if they were still present in the conversation history).


% Finally, we observed that interactions did not always follow the simple question-answer structure described in \Cref{sec:dialogues}, in which the programmer sought information and the wizard provided it. Sometimes wizards sought information from programmers (e.g. clarification questions); other times, programmers proactively offered information. Occasionally, a speaker would send multiple messages in a row, as demonstrated in the following excerpt:

% \vspace{-0.2cm}
% \begin{excerpt}
% \label{exc:followup}
% % \caption{An excerpt in which both the programmer and the wizard follow up on their own messages. Exchanges like this disrupt the typical pattern of question-answer pairs.  Messages are labeled with ``P'' or ``W'', denoting the speaker as a ``Programmer'' or ``Wizard,'' respectively.}
% \begin{tcolorbox}[left=5pt,right=-15pt,top=5pt,bottom=5pt]
% \begin{flushleft}
% \begin{dialogue}
% \speak{Pro} if I have an ALLEGRO\_EVENT called ev, should ev.type == ALLEGRO\_EVENT\_KEY\_DOWN return true when I press a key?
% \vspace{0.1cm}
% \speak{Wiz} I’m not sure I understand
% \vspace{0.1cm}
% \speak{Wiz} Are you interested in al\_get\_keyboard\_state or al\_key\_down?
% \vspace{0.1cm}
% \speak{Pro} no
% \vspace{0.1cm}
% \speak{Pro} tell me about al\_get\_keyboard\_state
% \end{dialogue}
% \end{flushleft}
% \end{tcolorbox}
% \label{exc:followup}
% \end{excerpt}
% \vspace{-0.2cm}

% In total, $15.7\%$ of the wizards' messages and $18.3\%$ of the programmers' messages were followed by one or more messages from that speaker.

Finally, we observed that speakers often expressed multiple, separate ideas and intentions within a single message. Identifying these separate utterances and parsing their meanings are key challenges a virtual assistant needs to overcome. The next section describes the first steps we've taken towards tackling these challenges. 
% Furthermore, speakers often expressed multiple, separate ideas and intentions within a single message. Identifying these separate utterances and parsing their meanings are key challenges a virtual assistant needs to overcome. The next section describes the first steps we've taken towards tackling these challenges. 

\vspace{-0.1cm}









\iffalse
\vspace{-0.2cm}
\subsection{Task Completion}
%A key factor in building a VA is an understaniding of optial wiz strats

%Task completion
Not every programmer completed every task. Task completion depended on a number of factors, including the programmer's and the wizard's skill. Recall that we hired 6 wizards; these wizards used a variety of strategies when assisting the programmers. As Reiser and Lemon~\cite{rieser2011reinforcement} describe, it is often best to study these strategies to discover which ones are optimal in which contexts. While this extensive analysis is beyond the scope of this paper, we present the programmers' task completion rates in order to characterize the corpus and provide direction for future work.



% Task completion depended on a number of factors, including programmer skill
%Not every prog completed every task
%task complete depends on both prog and wiz skill
%Recall we hired 6 wizs, each using a variety of strats
%as reiser and lemon point out, its iften best to study strats to find optimal ones

%Analyzing effects is more hard future work
%We present these rates to characterize ds and hint at future work
% Notice th

%

%Naturally, the programmers worked at different speeds and had different levels of success on the tasks.  
Specifically, we present two metrics: the task \emph{attempt rate} and the task \emph{completion rate}. We considered a programmer to have ``attempted'' a task if he or she wrote at least one line of code directly related to the task. If the relationship was ambiguous, we referred to the dialogue for additional context. We considered a programmer to have ``completed'' a task if, in our judgment, he or she wrote all of the code to satisfy all of the task's requirements, even if the code did not compile or execute. The following table shows programmers' attempt and completion rates for each task. For instance, $71.4\%$ of all programmers attempted Task D of the LibSSH scenario; of those programmers, $40.1\%$ completed the task.

\vspace{-0.2cm}
\begin{savenotes}
	\begin{table}[h!]
	% \caption{Programmers' performance on the tasks. ``Attempt rate'' refers to the percentage of all programmers that wrote at least one line code directly related to the task. ``Success rate'' refers to the percentage of all programmers that successfully completed the task.}
		\centering
		\begin{tabular}{lcrr}
			\toprule
			Scenario & Task                & Attempt Rate (\%)              & Completion Rate (\%)\\ 
			\midrule
			\multirow{5}{*}{LibSSH\footnote{Only 14 studies are considered here, as one participant in the LibSSH studies did not submit a source code file.}}&A&$100.0$&$100.0$\\
			&B&$100.0$&$78.6$\\
			&C&$100.0$&$21.4$\\
			&D&$71.4$&$40.1$\\
			&E&$51.1$&$28.0$\\
			\midrule
			\multirow{7}{*}{Allegro}&A&$100.0$&$73.3$\\
			&B&$93.3$&$78.6$\\
			&C&$80.0$&$33.4$\\
			&D&$40.0$&$66.8$\\
			&E&$6.7$&$100.0$\\
			&F&$6.7$&$100.0$\\
			&G&$0.0$&N/A\\
					\bottomrule
		\end{tabular}
		\label{tab:performance}
	\end{table}
\end{savenotes}{}
\vspace{-0.2cm}

Attempt and completion rates for different tasks varied between $0\%$ and $100\%$.  We generally observed lower attempt and completion rates for the later tasks, which were more difficult and for which the programmers may have had less time, depending on their performance on earlier tasks. Tasks E and F of the Allegro scenario each have a success rate of $100\%$ because only one programmer attempted and completed those tasks.  Programmers generally finished one task before moving to the next; however, they occasionally moved on from a task without successfully completing it.


%%Explain analaysis of wiz strats to demonstrate that we don't have space
%
% We note that task performance is not 
% We note that task performance is not necessarily a metric of programmer skill, as variations in the wizards affected the programmers' performance.
% While we leave detailed investigation into the roles of different factors on task performance as future work, for the time being, it is interesting to consider the dialogues in light of the programmers' performance. For instance, the worst-performing programmer in retrospect spent the majority of the interaction attempting to coax the full documentation out of Apiza, while the best-performing programmers asked specific questions, and upon encountering a dead-end (i.e. Apiza not being able to provide an answer), worked with Apiza to find a path forward. We make additional observations about programmer performance in \Cref{sec:obs}

\vspace{-0.2cm}
\subsection{User Satisfaction}

In addition to observing the programmers' objective performance on the tasks, we also asked programmers to fill out surveys subjectively rating their satisfaction with the ``virtual assistant'' system on a 5-point Likert scale.  These questions allow researchers to measure user satisfaction and evaluate wizard strategy, as well as train reinforcement learning algorithms for non-simulated dialogue systems (see \Cref{sec:woz}). The survey questions were inspired by the \texttt{PARADISE}~\cite{hajdinjak2006paradise} framework for automatic dialogue evaluation. To measure different dimensions of user satisfaction, the authors of the PARADISE framework created a set of 9 survey questions corresponding to features such as ``Interaction Pace'' and ``Task Ease.'' These questions have been widely adapted and used in subsequent dialogue studies~\cite{rieser2011reinforcement}. Although evaluation of the collected surveys is beyond the scope of this study, we present the survey questions and programmer responses in our online appendix.

% Although the original questions assumed spoken dialogue, the PARADISE authors noted that their framework could be applied to other modalities. The full set of questions we asked and the corresponding features are included in our online appendix.

 % It is our hope that these data will enable future researchers to evaluate the quality of different VA strategies and provide a baseline against which future dialogue systems can be compared.

% The features corresponding to the system's ability to understand user utterances (``Comprehension'') and the understandability of the system's utterances (``Comprehensibility'') were the most highly-rated, scoring around 4 points on average. The features related to the pace of the conversation (``Interaction Pace'') and the speed of the system's response (``System Response'') received the lowest ratings, around 3 points on average. Scores varied greatly across raters; the harshest rater gave an average score of 1.5, while the most generous rater awarded an average score of 4.9. 

% \vspace{-0.1cm}
% \begin{figure}[t]
%   \includegraphics[width=\linewidth]{figures/scores.png}
% 	\caption{Programmers' mean PARADISE scores for the Apiza system. Error bars show the 95\% confidence interval.}
%   \label{fig:DAdiff}
% \end{figure}
% \vspace{-0.1cm}

% That the features relating to interaction pace generally scored relatively low and those related to system understanding scored high is not surprising given the nature of the Wizard-of-Oz deception. For users accustomed to real virtual assistants, the system's high intelligence came as a pleasant surprise, while its sluggishness was a source of frustration.  As one programmer put it, ``Most of the time the first answer given by Apiza directly answered the question [...] The wait was a bit annoying though. I'm used to getting answers (well, search results) within a few seconds of entering a query.''

\vspace{-0.2cm}
\subsection{General Observations}
\label{sec:obs}

Overall, the programmers engaged well with the simulated system. Many programmers enjoyed interacting with Apiza and testing the system's capabilities, going so far as to ask questions like ``How's it going?'' and ``How is the weather where you are?'' Despite being allowed to search the internet for general C syntax questions, several programmers chose to direct these questions to Apiza. Conversely, a small number of programmers grew frustrated by Apiza's inability to provide certain information and decided to search for API documentation online. These violations were few and far between, and did not diminish the overall quality of the corpus.

In the dialogues, we observed habits that programmers may have learned by interacting with other virtual assistants and tools. Several programmers avoided the use of pronouns to refer to recently mentioned API components. They may have wanted to be as clear as possible in the event that Apiza would be unable to resolve the antecedent. Some programmers treated Apiza like a search engine, simply querying vagues terms without specifying the type of information desired. Many exhibited the ``Google Effect''~\cite{Sparrow776}: they would ask for previously established pieces of information (even if they were still present in the conversation history).

As noted in \Cref{sec:dialogues}, the interactions in the dialogues typically followed a simple question-answer structure, in which the programmer sought information and the wizard provided it. This was not always the case, however. Sometimes wizards sought information from the programmer (e.g. clarification questions); other times, programmers proactively offered information. Occasionally, a speaker would send multiple messages in a row, as demonstrated in the following excerpt:

\vspace{-0.2cm}
\begin{excerpt}
\label{exc:followup}
% \caption{An excerpt in which both the programmer and the wizard follow up on their own messages. Exchanges like this disrupt the typical pattern of question-answer pairs.  Messages are labeled with ``P'' or ``W'', denoting the speaker as a ``Programmer'' or ``Wizard,'' respectively.}
\begin{tcolorbox}[left=5pt,right=-15pt,top=5pt,bottom=5pt]
\begin{flushleft}
\begin{dialogue}
\speak{Pro} if I have an ALLEGRO\_EVENT called ev, should ev.type == ALLEGRO\_EVENT\_KEY\_DOWN return true when I press a key?
\vspace{0.1cm}
\speak{Wiz} I’m not sure I understand
\vspace{0.1cm}
\speak{Wiz} Are you interested in al\_get\_keyboard\_state or al\_key\_down?
\vspace{0.1cm}
\speak{Pro} no
\vspace{0.1cm}
\speak{Pro} tell me about al\_get\_keyboard\_state
\end{dialogue}
\end{flushleft}
\end{tcolorbox}
\label{exc:followup}
\end{excerpt}
\vspace{-0.2cm}

In total, $15.7\%$ of the wizards' messages and $18.3\%$ of the programmers' messages were followed by one or more messages from that speaker. Furthermore, speakers often expressed multiple, separate ideas and intentions within a single message. Identifying these separate utterances and parsing their meanings are key challenges a virtual assistant needs to overcome. The next section describes the first steps we've taken towards tackling these challenges. 

\fi





%Maybe don't discus
% We were curious to see if the extent of programmer-wizard interaction affected the programmers' task performance or satisfaction with the system. We hypothesized that programmers who had more interaction with the wizard would generally perform better at the tasks and have a more favorable opinion of the system. To test this, we considered the 

% While considering the programmers' performance and satisfaction, 

% *Discuss correlations between interaction and user performance and satisfaction

% *Discuss correlations between performance and satisfaction.
% We were curious to see if there were any clear correlations between the amount of interaction and performance or satisfaction. Answer: not really. Maybe a little. 

% However, there was relatively strong correlation between performance and satisfaction. Does not imply causality! But useful to know.


% As noted in \Cref{sec:dialogues}, the interactions in the dialogues typically followed a simple question-answer structure in which the programmers sought information and the wizards provided it. This was not always the case, however. Sometimes wizards sought information from the programmer (e.g. clarification questions); other times, programmers proactively offered information before posing a question. Occasionally, a speaker would send multiple messages in a row: $15.7\%$ of the wizards' messages and $18.3\%$ of the programmers' messages were followed by one or more messages from that speaker. This pattern occurred for a variety of reasons. Often, programmers would send a follow up message if the wizard was taking a long time to respond. Generally these messages would repeat or rephrase a prior question, or introduce a new question. Wizards would most frequently send multiple messages in a row when responding to a backlog of ananswered questions. Wizards and programmers both would occasionally follow up an answer or assesment with a new question, suggestion, offer, or repair, as shown in \Cref{exc:followup}.

% Conversations were relatively complex. Speakers sometimes sent multiple messages in a row, as shown in \Cref{exc:followup}. Even within a message, speakers expressed multiple intentions. This is one of the challenges a VA faces. Need to learn to identify intents etc- next section all about it.





